When Skills Fail to Compose: Compatibility and Retention in Language Models

Skill acquisition alone does not establish a reusable skill library: task proficiency does not specify a compositional interface. Motivated by agents that acquire and refine skills, we study independently learned soft-prompt skills on frozen language models, with skill identities and execution order supplied. Across four digit-task bases and three record-editing models, mean composition accuracy in one call is at most 7.6%, compared with 88.2% to 100% over two calls that add computation and an explicit intermediate output. Neutral-insertion training improves robustness but leaves substantial interference, which block length and per-token norm alone cannot explain on two of four digit bases. Blocks of the same operation need not be interchangeable: after training next to frozen learned partners, a post hoc test on two Qwen bases shows that replacing those partners with independently learned blocks of the same operations lowers median composition accuracy from 98.0% and 95.3% to 12.7% and 0.5%, although every replacement scores at least 90% alone. Repair can improve a composition while impairing the original skill, and rehearsal improves retention while transfer remains limited on Qwen2.5-0.5B. Internal interventions constrain explanations without identifying a shared failure mechanism. These findings motivate evaluating compatibility, retention and transfer alongside acquisition when building skill libraries for self-evolving agents. Code is available at https://github.com/YanLin-Quinne/SkillCompatibility.

==> figures/app_carrier_float.tex <==

\begin{figure*}[!t]
\centering
\includegraphics[width=\textwidth]{figures/app_carrier_v9.pdf}
\caption{\textbf{Soft blocks interfere on every eligible pair, while documents help mainly on 7B different-field pairs.} Panels give two-call-minus-one-call gaps in points for 0.5B, 1.5B and 7B, with blue soft blocks, purple invoked-only documents, grey dots for all six documents and a grey 10-point equivalence band.}
\label{fig:app-carrier}
\end{figure*}


==> figures/app_matrix_float.tex <==

\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{figures/app_matrix_v9.pdf}
\caption{\textbf{Directed-pair one-call accuracy is low on all four digit bases, with few exceptions.} Masked exact match (\%) over three seeds. Panel titles give the mean over the 27 non-degenerate pairs, hatched cells are excluded degeneracies, boxed cells non-commuting pairs and gray diagonal cells not pairs.}
\label{fig:app-matrix}
\end{figure*}


==> figures/fig_ha_float.tex <==


\begin{figure*}[!t]
\centering
\includegraphics[width=\textwidth]{figures/fig_ha_v9.pdf}
\caption{\textbf{Small head sets are rarely necessary, keep their attention after the gap and do not restore composition.} Green marks units with a qualifying $k^*$, gray dotted lines are random-set controls and shaded bands mark the specified ranges. In (b), dots are attention ratios (left axis) and dashes are $A$ presence (right axis).}
\label{fig:fig_ha}
\end{figure*}


==> figures/successor_distance_float.tex <==


\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{figures/successor_distance_v9.pdf}
\caption{\textbf{Earlier-skill presence under insertions and position gaps.} Medians at twenty positions (a, left) and by span length (b, right), with dashed lines at the 20\% and 80\% presence thresholds. 7B uses seeds 2 and 3.}
\label{fig:successor}
\end{figure*}


==> tables/app_ablation_seeds.tex <==
\begin{tabular}{@{}llcccccccccc@{}}
\toprule
\hlheadrow  & & \multicolumn{4}{c}{\hlhd{Composed accuracy}} & \multicolumn{4}{c}{\hlhd{Edited skill alone}} & \multicolumn{2}{c}{\hlhd{Holm $p$}} \\
\cmidrule(lr){3-6}\cmidrule(lr){7-10}\cmidrule(l){11-12}
\hlheadrow \hlhd{Base} & \hlhd{Seed} & \hlhd{$B$ anch.} & \hlhd{$B$ plain} & \hlhd{$A$ anch.} & \hlhd{$A$ plain} & \hlhd{$B$ anch.} & \hlhd{$B$ plain} & \hlhd{$A$ anch.} & \hlhd{$A$ plain} & \hlhd{side} & \hlhd{anchor} \\
\midrule
0.5B & 1 & \hlbest{70.0} & 52.3 & \hlbest{69.3} & 45.7 & \hlpass \hlbest{98.9} & \hlfail 16.7 & \hlpass \hlbest{98.4} & \hlfail 7.6 & \hlfail 1 & \hlfail 0.22 \\
0.5B & 2 & \hlbest{50.3} & 46.7 & \hlbest{44.3} & 35.3 & \hlpass \hlbest{97.6} & \hlfail 22.0 & \hlpass \hlbest{97.1} & \hlfail 4.7 & \hlfail 0.63 & \hlfail 0.35 \\
0.5B & 3 & \hlbest{57.7} & 18.3 & \hlbest{54.0} & 17.0 & \hlkey \hlbest{99.0} & \hlfail 4.9 & \hlpass \hlbest{97.7} & \hlfail 9.2 & \hlfail 1 & \hlpass 0.0021 \\
\addlinespace[2pt]
1.5B & 1 & 13.3 & \hlbest{16.3} & \hlbest{6.3} & 4.0 & \hlpass \hlbest{96.6} & \hlfail 4.3 & \hlkey \hlbest{88.9} & \hlfail 2.4 & \hlfail 0.68 & \hlfail 1 \\
1.5B & 2 & \hlbest{5.7} & \hlbest{5.7} & 6.0 & \hlbest{6.7} & \hlpass \hlbest{91.0} & \hlkey 0.9 & \hlpass \hlbest{91.4} & \hlfail 2.0 & \hlfail 1 & \hlfail 1 \\
1.5B & 3 & 7.0 & \hlbest{8.0} & 7.3 & \hlbest{9.3} & \hlpass \hlbest{92.8} & \hlfail 3.1 & \hlpass \hlbest{91.2} & \hlfail 5.6 & \hlfail 1 & \hlfail 1 \\
\addlinespace[2pt]
Gemma & 1 & \hlbest{35.0} & 24.3 & \hlbest{39.7} & 29.0 & \hlpass \hlbest{92.4} & \hlfail 1.2 & \hlpass \hlbest{92.4} & \hlfail 3.2 & \hlfail 1 & \hlpass 0.019 \\
Gemma & 2 & \hlbest{20.0} & 11.0 & \hlbest{26.3} & 18.0 & \hlpass \hlbest{90.2} & \hlfail 2.0 & \hlpass \hlbest{92.6} & \hlfail 19.8 & \hlfail 1 & \hlfail 0.37 \\
Gemma & 3 & \hlbest{38.7} & 36.7 & 48.7 & \hlbest{49.0} & \hlpass \hlbest{94.9} & \hlfail 4.9 & \hlpass \hlbest{91.2} & \hlfail 12.3 & \hlfail 0.62 & \hlfail 0.32 \\
\addlinespace[2pt]
7B & 2 & 9.3 & \hlbest{15.0} & \hlbest{18.3} & 15.0 & \hlpass \hlbest{97.4} & \hlkey 23.0 & \hlpass \hlbest{95.8} & \hlfail 8.8 & \hlfail 1 & \hlfail 0.62 \\
7B & 3 & \hlbest{7.0} & \hlbest{7.0} & 13.0 & \hlbest{15.7} & \hlpass \hlbest{97.1} & \hlfail 19.1 & \hlpass \hlbest{93.4} & \hlfail 10.6 & \hlfail 1 & \hlfail 1 \\
\addlinespace[2pt]
7B & 1$^\dagger$ & \hlbest{95.3} & 93.0 & 93.3 & \hlbest{95.7} & \hlpass \hlbest{99.9} & \hlfail 14.8 & \hlpass \hlbest{99.3} & \hlfail 4.0 & -- & -- \\
\bottomrule
\end{tabular}


==> tables/app_ablation_seeds_float.tex <==

\begin{table*}[!htbp]
\centering
\footnotesize
\setlength{\tabcolsep}{3.6pt}
\hlclip{\input{tables/app_ablation_seeds.tex}}
\caption{\textbf{Similar composition accuracy coexists with very different retention, and anchored editing keeps the edited skill at 88.9\% or above in every seed.} Medians (\%) over 27 digit pairs at eight composed labels, with one-sided Holm $p$ for the edit side and the anchor. $\dagger$: 7B seed 1, whose \sk{MOD3} fails, at 64 labels. Without labels, 0.5B composes 0.0\% with original and 0.3\% with layout-augmented skills.}
\label{tab:app-ablation-seeds}
\end{table*}


==> tables/app_accept_sens.tex <==


\hlclip{\begin{tabular}{@{}llcccccccc@{}}
\toprule
\hlheadrow  & & & & \multicolumn{3}{c}{\hlhd{Masked}} & \multicolumn{3}{c}{\hlhd{Unmasked}} \\
\cmidrule(lr){5-7}\cmidrule(l){8-10}
\hlheadrow \hlhd{Base} & \hlhd{Rule} & \hlhd{Cells} & \hlhd{Pairs} & \hlhd{One call} & \hlhd{Indep.} & \hlhd{Below} & \hlhd{One call} & \hlhd{Indep.} & \hlhd{Below} \\
\midrule
Qwen2.5-0.5B & all, length 8 & 81/81 & 27 & \hlkey 6.8 & 100.0 & \hlfail \hlbest{80/81} & 1.0 & 0.9 & 2/81 \\
\hlctrlrow  & pre-specified & 0/81 & 0 & -- & -- & -- & -- & -- & -- \\
 & revised & 61/81 & 27 & 8.5 & 100.0 & \hlfail \hlbest{60/61} & 1.3 & 1.2 & 2/61 \\
\midrule
Qwen2.5-1.5B & all, length 8 & 81/81 & 27 & 1.8 & 100.0 & \hlfail \hlbest{81/81} & 1.2 & 11.2 & 43/81 \\
 & pre-specified & 39/81 & 17 & 0.7 & 100.0 & \hlfail \hlbest{39/39} & 0.4 & 11.7 & 24/39 \\
 & revised & 55/81 & 27 & 1.2 & 100.0 & \hlfail \hlbest{55/55} & 0.8 & 15.5 & 35/55 \\
\midrule
Qwen2.5-7B & all cells & 81/81 & 27 & \hlkey 1.1 & 88.5 & \hlfail \hlbest{81/81} & 1.1 & 88.5 & 81/81 \\
 & pre-specified & 17/81 & 13 & 0.4 & 99.9 & \hlfail \hlbest{17/17} & 0.4 & 99.9 & 17/17 \\
 & revised & 43/81 & 25 & 0.7 & 99.9 & \hlfail \hlbest{43/43} & 0.7 & 99.9 & 43/43 \\
 & length 8 & 63/81 & 27 & 1.4 & 99.9 & \hlfail \hlbest{63/63} & 1.4 & 99.9 & 63/63 \\
\midrule
Gemma-3-1B & all, length 8 & 81/81 & 27 & 3.1 & 100.0 & \hlfail \hlbest{81/81} & 3.0 & 88.1 & 81/81 \\
 & pre-specified & 6/81 & 6 & 0.3 & 100.0 & \hlfail \hlbest{6/6} & 0.2 & 80.0 & 6/6 \\
 & revised & 71/81 & 27 & 3.4 & 100.0 & \hlfail \hlbest{71/71} & 3.3 & 87.1 & 71/71 \\
\bottomrule
\end{tabular}}

\medskip
\hlclip{\begin{tabular}{@{}lcccc@{}}
\toprule
\hlheadrow \hlhd{Masking check, 81 cells per base} & \hlhd{0.5B} & \hlhd{1.5B} & \hlhd{7B} & \hlhd{Gemma} \\
\midrule
Single skill with the library, masked / unmasked & 100.0 / 8.9 & 100.0 / 36.3 & 94.2 / 94.2 & 100.0 / 93.9 \\
Unmasked outputs emitting a skill token & 95.7 & 72.3 & 0.0 & 18.3 \\
Same content, masked and unmasked & 4.3 & 27.7 & 100.0 & 81.7 \\
\quad among unmasked outputs without a skill token & 100.0 & 100.0 & 100.0 & 100.0 \\
Installed alone, masked / unmasked & 100.0 / 100.0 & 100.0 / 100.0 & 94.0 / 94.0 & 100.0 / 100.0 \\
\bottomrule
\end{tabular}}


==> tables/app_accept_sens_float.tex <==

\begin{table*}[!htbp]
\centering
\footnotesize
\setlength{\tabcolsep}{4pt}
\input{tables/app_accept_sens.tex}
\caption{\textbf{Interference persists among accepted constituents, and masking changes outputs only on tied bases.} Accuracies in \%, ``Below'' counts cells significantly under the independence reference after Holm correction, ``all, length 8'' marks bases where the length-8 rule keeps every cell, and the lower block gives the masking checks.}
\label{tab:app-accept-sens}
\end{table*}


==> tables/app_acceptance.tex <==


\hlclip{\begin{tabular}{@{}lcccp{8.9cm}@{}}
\toprule
\hlheadrow \hlhd{Base} & \hlhd{Pre-spec.} & \hlhd{Revised} & \hlhd{Length 8} & \hlhd{Skills failing the revised rule by seed, length 8 / held-out 5 and 7} \\
\midrule
Qwen2.5-0.5B & 3/18 & 16/18 & 18/18 & s1 SWAP 100.0/59.0, s2 SWAP 100.0/50.0 \\
Qwen2.5-1.5B & 13/18 & 15/18 & 18/18 & s1 SWAP 100.0/83.3, s2 SR 100.0/88.7, SWAP 100.0/85.0 \\
Qwen2.5-7B & 9/18 & 13/18 & 16/18 & s1 SR 100.0/61.8, MOD3 3.0/28.5 $\dagger$, s2 SL 100.0/67.0, s3 IP 89.0/79.0, SL 100.0/87.3 \\
Gemma-3-1B & 5/18 & 17/18 & 18/18 & s3 SWAP 100.0/43.0 \\
\hlctrlrow Llama-3.2-1B & 1/18 & 1/18 & 2/18 & 17 of 18 fail, SR and MOD3 0.0 at length 8 in every seed, the only pass is IP in s3 \\
\bottomrule
\end{tabular}}


==> tables/app_acceptance_float.tex <==

\begin{table*}[t]
\centering
\footnotesize
\input{tables/app_acceptance.tex}

\medskip
\hlclip{\begin{tabular}{@{}lll@{}}
\toprule
\hlheadrow \hlhd{Measure} & \hlhd{Mistral-7B-v0.3} & \hlhd{Pre-specified rule} \\
\midrule
Digit base, bf16 pretraining & \hlpass full schedule, no NaN & stop on any NaN \\
Base: one pretrained op, length 8 & \hlpass 100.0 & at least 90\% \\
Base: two and three ops, length 8 & 90.0 and 82.0 & descriptive \\
Skills alone, revised rule, seed 1 & \hlfail 0 of 6 & stop if 2 or more of 6 fail \\
Skills alone, revised rule, all seeds & 4 of 18 & reported \\
Skills alone, pre-specified rule, all seeds & 0 of 18 & reported \\
Skills alone, at least 90\% at length 8 & 12 of 18 & descriptive \\
Layout-augmented skills, revised rule & 1 of 18 & descriptive \\
\hlctrlrow One call and every control & run, not used & stop rule \\
\bottomrule
\end{tabular}}
\caption{\textbf{The revised rule accepts most skill seeds on every included base, while the Mistral extension stops at its skill gate.} Upper block: unmasked accuracy of each skill installed alone, with the skill seeds passing each rule or reaching 90\% at length 8, the failing skills by seed (s1 to s3) with length-8 / held-out scores (\%), and $\dagger$ the compromised 7B seed. The released code reproduces the per-skill Llama scores. Lower block: Mistral-7B-v0.3 against its pre-specified rules (\%).}
\label{tab:app-acceptance}
\end{table*}


==> tables/app_c1.tex <==


\begin{tabular}{@{}lccccc@{}}
\toprule
\hlheadrow  & & & \multicolumn{3}{c}{\hlhd{Gap}} \\
\cmidrule(lr){4-6}
\hlheadrow \hlhd{Condition} & \hlhd{Single} & \hlhd{One call} & \hlhd{D} & \hlhd{S} & \hlhd{T} \\
\midrule
Text, full & 97.7 & \hlbest{70.2} & \hlbest{3.8} & \hlbest{9.6} & 62.7 \\
Text, procedure & 80.3 & 43.2 & 46.4 & 19.3 & \hlbest{60.1} \\
Text, examples & 95.5 & 54.2 & 13.1 & 38.4 & 86.0 \\
\midrule
Soft & \hlbest{99.5} & 2.0 & 97.8 & 91.8 & 99.9 \\
Soft, examples & 83.1 & 22.4 & 71.5 & 71.7 & 96.9 \\
Soft, examples, ids & 84.7 & 28.4 & 62.1 & 73.3 & 93.9 \\
\midrule
Text + soft blocks & 92.8 & 57.8 & 20.3 & 11.2 & 73.8 \\
Text + random & 98.1 & 68.5 & 3.7 & 18.0 & 63.0 \\
Text + norm-matched & 97.8 & 67.7 & 4.7 & 17.8 & 64.0 \\
\quad draw 2 & 98.0 & 68.9 & 4.2 & 15.9 & 61.4 \\
\quad draw 3 & 98.1 & 67.9 & 4.9 & 16.2 & 64.2 \\
\midrule
Text, 20 tokens each & 79.6 & 17.8 & 91.2 & 79.9 & 52.5 \\
\quad single, NI / SC & \multicolumn{5}{l}{76.0 / 7.7} \\
Soft with names & 79.9 & 11.2 & 86.1 & 91.2 & 90.0 \\
Names only & 27.7 & 2.1 & 97.1 & 97.5 & 95.9 \\
\bottomrule
\end{tabular}


==> tables/app_c1_float.tex <==


\begin{table}[!t]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\hlclip{\input{tables/app_c1.tex}}
\caption{\textbf{Examples support document composition, terse text and names fail, and trained blocks harm 8 of 18 pairs versus 1 for random blocks.} Means over three draws or seeds on 7B, accuracies in \%, gaps in points for different-field (D), same-name-field (S) and same-total (T) pairs. ``ids'' marks examples labelled by soft-skill ID, and bold the best value per column in the first two panels.}
\label{tab:app-c1}
\end{table}


==> tables/app_cost.tex <==


\begin{tabular}{@{}llccccc@{}}
\toprule
\hlgrouprow \multicolumn{7}{@{}l}{\emph{Serving, per request (batched, and batch 1 on 0.5B)}} \\
\hlheadrow \hlhd{Base} & & \hlhd{One call, ms} & \hlhd{Two calls, ms} & \hlhd{Prompt tokens} & \hlhd{Accuracy} & \hlhd{Batch 1, ms} \\
\midrule
Qwen2.5-0.5B & & 12.2 & 23.8 & 49/58 & 6.4/100.0 & 457 / 913 \\
Qwen2.5-1.5B & & 12.7 & 23.0 & 49/58 & 1.3/99.9 & -- \\
Qwen2.5-7B & & 15.9 & 26.6 & 49/58 & 0.9/88.2 & -- \\
Gemma-3-1B & & 17.6 & 34.2 & 49/58 & 2.7/100.0 & -- \\
\midrule
\hlgrouprow \multicolumn{7}{@{}l}{\emph{One-off training per pair, main budget files (8-label rows for 0.5B only)}} \\
\hlheadrow \hlhd{Base} & \hlhd{Method} & \hlhd{Labels} & \hlhd{Accuracy} & \hlhd{Train s [IQR]} & \hlhd{Break-even} & \hlhd{Batch 1} \\
\midrule
Qwen2.5-0.5B & anchored & 8 & 55.0 & 51 [48, 57] & 4394 & 112 \\
Qwen2.5-0.5B & anchored & 64 & 100.0 & 129 [124, 135] & 11115 & 283 \\
Qwen2.5-0.5B & SPoT & 8 & 42.7 & 49 [47, 54] & 4222 & 108 \\
Qwen2.5-0.5B & SPoT & 64 & 100.0 & 146 [134, 152] & 12580 & 320 \\
Qwen2.5-1.5B & anchored & 64 & 98.0 & 166 [156, 173] & 16230 & -- \\
Qwen2.5-1.5B & SPoT & 64 & 97.0 & 165 [154, 171] & 16084 & -- \\
Qwen2.5-7B & anchored & 64 & 93.7 & 133 [128, 140] & 12412 & -- \\
Qwen2.5-7B & SPoT & 64 & 90.7 & 135 [131, 140] & 12598 & -- \\
Gemma-3-1B & anchored & 64 & 98.7 & 204 [196, 219] & 12309 & -- \\
Gemma-3-1B & SPoT & 64 & 99.0 & 206 [194, 221] & 12400 & -- \\
\bottomrule
\end{tabular}


==> tables/app_cost_float.tex <==

\begin{table*}[!htbp]
\centering
\footnotesize
\setlength{\tabcolsep}{2.6pt}\renewcommand{\arraystretch}{1.25}
\hlclip{\input{tables/app_cost.tex}}
\caption{\textbf{One-call repair saves latency but amortises its training only over many requests.} Accuracy (\%) is the median over pairs of medians over timed skill seeds, and break-even counts compare only within a base. The released code reproduces the eight-label rows of the other bases.}
\label{tab:app-cost}
\end{table*}


==> tables/app_failure.tex <==


\hlclip{\begin{tabular}{@{}lccccccccc@{}}
\toprule
\hlheadrow \hlhd{Base} & \hlhd{$B(A(x))$} & \hlhd{$B(x)$} & \hlhd{$A(x)$} & \hlhd{$x$} & \hlhd{Short} & \hlhd{Format} & \hlhd{Partial} & \hlhd{Shift} & \hlhd{Other} \\
\midrule
Qwen2.5-0.5B & 6.8 & 10.8 & 0.8 & 0.2 & 18.9 & 0.0 & 11.0 (4.5) & 0.2 & 51.3 (76.1) \\
Qwen2.5-1.5B & 1.8 & \hlkey 12.0 & 3.7 & 4.5 & 11.8 & 0.3 & 6.0 (4.2) & 0.1 & 59.9 (83.3) \\
Qwen2.5-7B & 1.1 & \hlkey 8.5 & 4.6 & 3.3 & 7.2 & 3.0 & 5.4 (4.2) & 0.1 & 66.8 (85.3) \\
Gemma-3-1B & 3.1 & 9.0 & 0.9 & 4.5 & 19.6 & 0.8 & 8.7 (3.3) & 0.1 & 53.3 (76.0) \\
\bottomrule
\end{tabular}}

\vspace{6pt}

\hlclip{\begin{tabular}{@{}lcccccc@{}}
\toprule
 & \multicolumn{3}{c}{\hlhd{Masked}} & \multicolumn{3}{c}{\hlhd{Unmasked}} \\
\cmidrule(lr){2-4}\cmidrule(l){5-7}
\hlheadrow \hlhd{Base} & \hlhd{First lost} & \hlhd{Second lost} & \hlhd{First ahead} & \hlhd{First lost} & \hlhd{Second lost} & \hlhd{First ahead} \\
\midrule
Qwen2.5-0.5B & $+$23.6 & $-$6.4 & 18/27 (0.12) & $+$25.5 & $-$10.5 & 21/27 (0.0059) \\
Qwen2.5-1.5B & $+$15.2 & $-$2.4 & 16/27 (0.44) & $+$20.5 & $-$2.9 & 17/27 (0.25) \\
Qwen2.5-7B & $+$14.0 & $-$2.6 & 17/27 (0.25) & $+$14.0 & $-$2.6 & 17/27 (0.25) \\
Gemma-3-1B & $+$13.7 & $-$11.4 & 17/27 (0.25) & $+$14.8 & $-$12.1 & 18/27 (0.12) \\
\bottomrule
\end{tabular}}


==> tables/app_failure_float.tex <==

\begin{table*}[!htbp]
\centering
\footnotesize
\setlength{\tabcolsep}{3.4pt}
\input{tables/app_failure.tex}
\caption{\textbf{Most digit outputs match no exact error class.} Upper-panel shares (\%) over all evaluation items pool three seeds with chance in parentheses, lower-panel values are post hoc excess over chance in points with sign-test $p$, and yellow marks quoted~values.}
\label{tab:app-failure}
\end{table*}


==> tables/app_l1.tex <==
\begin{tabular}[t]{@{}l@{}}\textbf{(a) Pairwise composition}\\[2pt]
\hlclip{\begin{tabular}[t]{@{}lcc@{}}
\toprule
\hlheadrow & \hlhd{Layout-} & \\
\hlheadrow \hlhd{Pair} & \hlhd{augmented} & \hlhd{Original} \\
\midrule
SL$\to$IP & \hlbest{36.3} & 0.7 \\
IP$\to$SR & 13.3 & \hlbest{88.3} \\
MIRROR$\to$SR & \hlbest{12.3} & 0.7 \\
SWAP$\to$IP & \hlbest{7.3} & 6.7 \\
IP$\to$SWAP & \hlbest{6.3} & \hlbest{6.3} \\
MOD3$\to$SR & 6.0 & \hlbest{15.7} \\
SR$\to$IP & \hlbest{5.7} & 1.7 \\
IP$\to$SL & 4.0 & \hlbest{10.7} \\
MOD3$\to$SL & \hlbest{3.3} & 0.7 \\
SR$\to$MOD3 & \hlbest{2.0} & 0.0 \\
SWAP$\to$MOD3 & 0.3 & \hlbest{0.7} \\
MOD3$\to$IP & 0.3 & \hlbest{1.7} \\
MOD3$\to$SWAP & \hlbest{0.3} & \hlbest{0.3} \\
MIRROR$\to$MOD3 & \hlbest{0.3} & 0.0 \\
SR$\to$SWAP & 0.0 & 0.0 \\
SR$\to$MIRROR & 0.0 & 0.0 \\
IP$\to$MIRROR & 0.0 & 0.0 \\
SL$\to$SWAP & 0.0 & 0.0 \\
SL$\to$MOD3 & 0.0 & 0.0 \\
SL$\to$MIRROR & 0.0 & 0.0 \\
SWAP$\to$SR & 0.0 & 0.0 \\
SWAP$\to$SL & 0.0 & 0.0 \\
SWAP$\to$MIRROR & 0.0 & 0.0 \\
MOD3$\to$MIRROR & 0.0 & 0.0 \\
MIRROR$\to$IP & 0.0 & \hlbest{97.0} \\
MIRROR$\to$SL & 0.0 & 0.0 \\
MIRROR$\to$SWAP & 0.0 & 0.0 \\
Median & \hlkey \hlbest{0.3} & 0.0 \\
Mean & 3.6 & \hlbest{8.6} \\
\bottomrule
\end{tabular}}
\end{tabular}\hspace{18pt}
\begin{tabular}[t]{@{}l@{}}\textbf{(b) Earlier-skill presence and classifications}\\[2pt]
\hlclip{\begin{tabular}[t]{@{}lccc@{}}
\toprule
\hlheadrow & & \hlhd{Layout-} & \\
\hlheadrow \hlhd{After $A$} & \hlhd{Positions} & \hlhd{augmented} & \hlhd{Original} \\
\midrule
random rows, 1 & 1 & \hlpass \hlbest{100.0} & 25.8 \\
random rows, 5 & 5 & \hlpass \hlbest{100.0} & 17.2 \\
random rows, 10 & 10 & \hlpass \hlbest{100.0} & 2.2 \\
random rows, 20 & 20 & \hlpass \hlbest{100.0} & 4.0 \\
random rows, 40 & 40 & \hlpass \hlbest{99.5} & 0.8 \\
\sk{INIT} rows, 20 & 20 & \hlpass \hlbest{100.0} & 11.0 \\
\sk{ID} copies, 1 & 2 & \hlpass \hlbest{100.0} & \hlbest{100.0} \\
\sk{ID} copies, 5 & 10 & \hlpass \hlbest{100.0} & 99.3 \\
\sk{ID} copies, 10 & 20 & \hlpass \hlbest{100.0} & 94.2 \\
\sk{ID} copies, 20 & 40 & \hlpass \hlbest{99.7} & 50.5 \\
\sk{ID} copies, 40 & 80 & \hlpass \hlbest{98.8} & 35.8 \\
` the' copies, 5 & 5 & \hlpass \hlbest{100.0} & 49.8 \\
` the' copies, 10 & 10 & \hlpass \hlbest{100.0} & 15.8 \\
` the' copies, 20 & 20 & \hlpass \hlbest{100.0} & 6.7 \\
` the' copies, 40 & 40 & \hlpass \hlbest{100.0} & 11.2 \\
gap, nothing inserted, 5 & 5 & \hlfail 0.0 & 0.0 \\
gap, nothing inserted, 10 & 10 & \hlfail 0.0 & 0.0 \\
gap, nothing inserted, 20 & 20 & \hlfail 0.0 & 0.0 \\
gap, nothing inserted, 40 & 40 & \hlfail 0.0 & 0.0 \\
\sk{REVERSE} & 4 & \hlpass \hlbest{100.0} & \hlbest{100.0} \\
trained $B$, cells $<$ 20\% & -- & 73/81 & 74/81 \\
trained $B$, pairs, most seeds & -- & 25/27 & 25/27 \\
Majority outcome & -- & gap only & gap and insertions \\
\bottomrule
\end{tabular}}
\end{tabular}


==> tables/app_l1_float.tex <==

\begin{table*}[!htbp]
\centering
\footnotesize
\setlength{\tabcolsep}{4pt}
\input{tables/app_l1.tex}
\caption{\textbf{Layout augmentation improves insertion robustness but not composition.} Qwen2.5-0.5B, masked decoding, values in \%: (a) one-call accuracy with the augmented skill first, as seed medians, and (b) median presence over 18 units with counts over 27 pairs and three seeds. Teal and coral cells meet the preservation and loss cut-offs, yellow is quoted in the main text and bold is the better nonzero value per row.}
\label{tab:app-l1}
\end{table*}


==> tables/app_l2.tex <==
\begin{tabular}{@{}lcccc@{}}
\toprule
\hlheadrow & \multicolumn{2}{c}{\hlhd{Qwen2.5-0.5B}} & \multicolumn{2}{c}{\hlhd{Qwen2.5-1.5B}} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
\hlheadrow \hlhd{Partner} & \hlhd{Comp.} & \hlhd{Kept} & \hlhd{Comp.} & \hlhd{Kept} \\
\midrule
\hlgrouprow \multicolumn{5}{@{}l}{\emph{Original partner rows (pre-specified)}} \\
Seen identity & \hlpass 98.0 & \hlpass 21 & \hlpass 95.3 & \hlpass 19 \\
Held-out identity & \hlfail 0.0 & \hlfail 2 & \hlfail 0.0 & \hlfail 1 \\
\midrule
\hlgrouprow \multicolumn{5}{@{}l}{\emph{New partner rows, seeds 104 and 105 (post hoc)}} \\
Seen identity & \hlfail 12.7 & \hlfail 3 & \hlfail 0.5 & \hlfail 1 \\
Held-out identity & \hlfail 0.0 & \hlfail 2 & \hlfail 0.0 & \hlfail 1 \\
\bottomrule
\end{tabular}


==> tables/app_l2_float.tex <==
\begin{table}[!htbp]
\centering
\footnotesize
\setlength{\tabcolsep}{4pt}
\hlclip{\input{tables/app_l2.tex}}
\caption{\textbf{Learned-partner gains appear mainly with the trained partner rows (new rows post hoc).} Comp.\ is median composition in \% and Kept counts pairs keeping $A$, teal meets the benchmark or bar and coral is below 20\% of the scale.}
\label{tab:app-l2}
\end{table}


==> tables/app_ll.tex <==
\begin{tabular}{@{}lccc@{}}
\toprule
\hlheadrow \hlhd{Rows per skill} & \hlhd{5} & \hlhd{20} & \hlhd{40} \\
\midrule
Gap of 20, max $A$ present & \hlfail 0.7 & \hlfail 0.3 & \hlfail 0.7 \\
20 random rows, max $A$ present & 37.0 & \hlfail 15.7 & \hlbest{76.7} \\
Gap $\ge$ 50\% & 0/6 & 0/6 & 0/6 \\
Gap and random rows $<$ 20\% & 5/6 & 6/6 & 4/6 \\
Units: gap and insertions, gap only & 5, 1 & 4, 2 & 4, 2 \\
Trained $B$, pairs $<$ 20\% & 27/27 & 26/27 & 25/27 \\
Single accuracy, min & \hlbest{100.0} & \hlbest{100.0} & \hlbest{100.0} \\
Joint accuracy, median & 0.0 & 0.0 & 0.0 \\
Joint accuracy, mean & 0.4 & 5.7 & \hlbest{8.5} \\
Pairs with joint $\ge$ 10\% & 0 & 4 & 6 \\
\bottomrule
\end{tabular}


==> tables/app_ll_float.tex <==
\begin{table}[!htbp]
\centering
\footnotesize
\setlength{\tabcolsep}{4pt}
\hlclip{\input{tables/app_ll.tex}}
\caption{\textbf{Fragility persists across 5-, 20- and 40-row skills.} Qwen2.5-0.5B, seed 1, values in \%, maxima over the six skills, counts over skills, units or the 27 pairs. Coral is below the loss cut-off and bold the best nonzero, non-coral value per row.}
\label{tab:app-ll}
\end{table}


==> tables/app_lr.tex <==

\begin{tabular}{@{}llcccccccc@{}}
\toprule
\hlheadrow  & & \multicolumn{2}{c}{\hlhd{0.5B}} & \multicolumn{2}{c}{\hlhd{1.5B}} & \multicolumn{2}{c}{\hlhd{7B}} & \multicolumn{2}{c}{\hlhd{Gemma}} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(l){9-10}
\hlheadrow \hlhd{Method} & \hlhd{lr} & \hlhd{4} & \hlhd{8} & \hlhd{4} & \hlhd{8} & \hlhd{4} & \hlhd{8} & \hlhd{4} & \hlhd{8} \\
\midrule
Anchored & 0.001 & 4.7 & 48.3 & 0.7 & 2.7 & 0.3 & 3.7 & 3.7 & 29.0 \\
Anchored & 0.005 & \textbf{6.3} & \textbf{70.0} & \textbf{0.3} & \textbf{13.3} & \textbf{0.0} & \textbf{4.7} & \textbf{3.3} & \textbf{35.0} \\
Anchored & 0.02 & 2.0 & 26.7 & 0.3 & 7.7 & 0.3 & 3.7 & 0.3 & 5.3 \\
\midrule
SPoT & 0.0003 & 1.7 & 12.3 & 0.3 & 0.7 & 0.0 & 1.0 & 3.3 & 13.0 \\
SPoT & 0.001 & \textbf{6.7} & \textbf{69.0} & \textbf{0.3} & \textbf{9.3} & \textbf{0.3} & \textbf{9.3} & \textbf{4.3} & \textbf{38.7} \\
SPoT & 0.005 & 1.7 & 26.7 & 0.7 & 6.0 & 0.3 & 2.7 & 0.0 & 4.0 \\
SPoT & 0.02 & 0.0 & 0.3 & 0.0 & 0.7 & 0.0 & 0.7 & 0.0 & 0.0 \\
\midrule
Connector & 0.0003 & -- & -- & 0.3 & 0.3 & 0.0 & 1.7 & -- & -- \\
Connector & 0.001 & 2.3 & 12.3 & \textbf{0.0} & \textbf{0.7} & \textbf{0.3} & \textbf{3.7} & 0.7 & 5.0 \\
Connector & 0.005 & 1.7 & 12.0 & 0.0 & 0.3 & 0.7 & 2.0 & \textbf{1.7} & \textbf{11.0} \\
Connector & 0.02 & \textbf{1.3} & \textbf{15.7} & 0.0 & 0.3 & 0.0 & 2.7 & 0.3 & 8.0 \\
Connector & 0.05 & 1.3 & 9.3 & -- & -- & -- & -- & -- & -- \\
\bottomrule
\end{tabular}


==> tables/app_lr_float.tex <==

\begin{table}[tp]
\centering
\footnotesize
\setlength{\tabcolsep}{2pt}
\hlclip{\input{tables/app_lr.tex}}
\caption{\textbf{Every selected learning rate is interior to its grid, and SPoT is the most rate-sensitive method.} Median composition accuracy (\%) over twenty-seven seed-1 pairs at four and eight labels, with selected rates in bold and untested ones dashed.}
\label{tab:app-lr}
\end{table}


==> tables/app_nb_summary_float.tex <==

\begin{table}[!htbp]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\hlclip{\begin{tabular}{@{}lcc@{}}
\toprule
\hlheadrow \hlhd{Qwen2.5-Instruct} & \hlhd{0.5B} & \hlhd{7B} \\
\midrule
Eligible units & 14/18 & 18/18 \\
\hlgrouprow \multicolumn{3}{@{}l}{\emph{$B$ present (\%) with $B$ alone}} \\
plain & 100.0 & 99.5 \\
after neutral prose & 81.1 & 37.7 \\
after ten \sk{ID} copies & 99.7 & 90.9 \\
after random rows & 85.4 & 87.5 \\
after \sk{INIT} rows & 92.6 & 74.1 \\
shifted by 4 positions & 100.0 & 99.5 \\
shifted by 20 positions & 100.0 & 98.8 \\
own block hidden, check & 0.0 & 0.0 \\
\hlgrouprow \multicolumn{3}{@{}l}{\emph{$B$ present (\%) after $A$}} \\
after soft $A$, one call & 18.1 & 9.7 \\
after the terse text of $A$ & 72.5 & 20.5 \\
prefix label & \hlpass \hlbest{soft} & \hlfail \hlbest{mixed} \\
\hlgrouprow \multicolumn{3}{@{}l}{\emph{One call (\%)}} \\
$B$, $A$ hidden from $B$'s block & 62.3 & 42.7 \\
$B$, $A$ hidden from later positions & 55.2 & 19.3 \\
$B$, $A$ hidden from both & 100.0 & 99.0 \\
$B$, system message hidden, control & \hlpass 18.0 & \hlpass 8.9 \\
$A$, $A$ hidden from later positions & \hlpass 0.0 & \hlpass 0.0 \\
both edits present & 5.5 & 1.5 \\
collapse share & 4.7 & 18.5 \\
knockout label & \hlfail \hlbest{mixed} & \hlpass \hlbest{joint} \\
\quad without collapsed cells & \hlfail \hlbest{mixed} & \hlfail \hlbest{mixed} \\
\hlgrouprow \multicolumn{3}{@{}l}{\emph{Band-limited knockout, gain in points}} \\
knockout & $B$'s block & both \\
full depth & 44.2 & 89.3 \\
first third & \hlpass \hlbest{39.4} & \hlfail \hlbest{43.7} \\
second third & 7.2 & 4.3 \\
third third & 0.2 & 0.5 \\
base reading & \hlbest{localized} & \hlbest{distributed} \\
units localized in the first third & 8/14 & 9/18 \\
\bottomrule
\end{tabular}}
\caption{\textbf{Language successors meet no combined signature on either base.} Means over eligible units, with teal marking a passed check, a majority label or a first third reaching half the full-depth gain and coral the~opposite.}
\label{tab:app-nb}
\end{table}


==> tables/app_neo_reverse.tex <==
\begin{tabular}{@{}lcccccc@{}}
\toprule
\hlheadrow & \multicolumn{3}{c}{\hlhd{Learned}} & \multicolumn{3}{c}{\hlhd{Pretrained}} \\
\hlheadrow & \multicolumn{3}{c}{\hlhd{\sk{NEO\_REVERSE}}} & \multicolumn{3}{c}{\hlhd{\sk{REVERSE}}} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
\hlheadrow \hlhd{Skill} & \hlhd{1} & \hlhd{2} & \hlhd{3} & \hlhd{1} & \hlhd{2} & \hlhd{3} \\
\midrule
\hlgrouprow \multicolumn{7}{@{}l}{\emph{Skill first: $A$ present after the block}} \\
SR & \hlfail 5.7 & \hlfail 0.0 & \hlfail 0.2 & \hlpass 99.8 & \hlpass 99.9 & \hlpass 100.0 \\
IP & \hlfail 18.0 & \hlpass 89.4 & \hlpass 87.5 & \hlpass 100.0 & \hlpass 100.0 & \hlpass 99.8 \\
SL & \hlfail 0.2 & \hlfail 0.2 & \hlfail 0.5 & \hlpass 99.8 & \hlpass 99.7 & \hlpass 99.7 \\
SWAP & \hlfail 0.0 & \hlfail 0.1 & \hlfail 0.2 & \hlpass 99.4 & \hlpass 98.9 & \hlpass 99.8 \\
MOD3 & \hlfail 0.0 & \hlfail 0.0 & \hlfail 0.0 & \hlpass 99.9 & \hlpass 100.0 & \hlpass 100.0 \\
MIRROR & \hlfail 0.2 & \hlfail 0.0 & \hlfail 0.0 & \hlpass 97.5 & \hlpass 97.0 & \hlpass 96.9 \\
\midrule
\hlgrouprow \multicolumn{7}{@{}l}{\emph{Block first: one-call exact match}} \\
SR & 0.0 & 0.0 & 0.0 & 100.0 & 100.0 & 100.0 \\
IP & 81.2 & 26.0 & 58.0 & 100.0 & 100.0 & 99.0 \\
SL & 0.4 & 4.0 & 0.1 & 100.0 & 99.0 & 99.0 \\
SWAP & 0.1 & 0.1 & 1.5 & 100.0 & 100.0 & 100.0 \\
MOD3 & 0.0 & 0.0 & 0.0 & 98.0 & 100.0 & 98.0 \\
MIRROR & 0.0 & 0.0 & 0.0 & 100.0 & 98.0 & 98.0 \\
\bottomrule
\end{tabular}


==> tables/app_neo_reverse_float.tex <==
\begin{table}[!htbp]
\centering
\footnotesize
\setlength{\tabcolsep}{4pt}
\hlclip{\input{tables/app_neo_reverse.tex}}
\caption{\textbf{Learned versus pretrained \sk{REVERSE} beside digit skills.} Post hoc, values in \%, columns are skill seeds, colors mark the 20\% and 80\% cut-offs.}
\label{tab:app-neo-reverse}
\end{table}


==> tables/app_nl_mech.tex <==
\begin{tabular}[t]{@{}l@{}}\textbf{(a) Skill effects by pair class and over skills}\\[2pt]
\hlclip{\begin{tabular}[t]{@{}lccc@{}}
\toprule
\hlheadrow & \hlhd{0.5B} & \hlhd{1.5B} & \hlhd{7B} \\
\midrule
\hlgrouprow \multicolumn{4}{@{}l}{\emph{One call: earlier / later skill applied}} \\
\quad different fields & 57.1 / 19.0 & 58.9 / 13.5 & 70.3 / 9.7 \\
\quad same name field & 46.1 / 18.2 & 45.8 / 0.2 & 80.6 / 9.3 \\
\quad same total & 75.6 / 33.4 & 78.0 / 19.6 & 65.9 / 12.1 \\
\quad all thirty pairs & 58.6 / 21.7 & 60.1 / 12.1 & 71.5 / 10.1 \\
\quad output parses & 95.3 & 99.7 & 81.9 \\
\hlgrouprow \multicolumn{4}{@{}l}{\emph{Mean over skills}} \\
\quad mean loss, first / second & 39.3 / 76.1 & 38.3 / 86.3 & 28.5 / 89.9 \\
\quad $B$ on the gold intermediate & 5/6 $\ge$ 99.9 & 5/6 $\ge$ 99.9 & 5/6 $\ge$ 99.9 \\
\bottomrule
\end{tabular}}
\end{tabular}\hspace{12pt}
\begin{tabular}[t]{@{}l@{}}\textbf{(b) Prefix and order controls}\\[2pt]
\hlclip{\begin{tabular}[t]{@{}lccc@{}}
\toprule
\hlheadrow & \hlhd{0.5B} & \hlhd{1.5B} & \hlhd{7B} \\
\midrule
\hlgrouprow \multicolumn{4}{@{}l}{\emph{$A$ present minus $A$ alone}} \\
\quad \sk{ID} after $A$ & 0.0 & $-$0.1 & $-$0.1 \\
\quad \sk{ID} before $A$ & $-$0.1 & $-$0.6 & $-$0.2 \\
\quad \sk{INIT} block after $A$ & $-$0.1 & $-$16.6 & $-$9.2 \\
\quad neutral text after $A$ & $-$0.7 & $-$30.2 & $-$10.2 \\
\quad random block after $A$ & $-$4.0 & $-$19.1 & $-$3.1 \\
\quad random block before $A$ & $-$17.4 & $-$50.8 & $-$12.1 \\
\quad text instruction for $B$ after $A$ & $-$8.6 & $-$53.2 & $-$50.7 \\
\hlgrouprow \multicolumn{4}{@{}l}{\emph{Later skill applied, by what separates the two}} \\
\quad nothing & 21.7 & 12.1 & 10.1 \\
\quad \sk{ID} & 22.6 & 15.6 & 10.9 \\
\quad the word ``then'' & 24.6 & 15.0 & 12.1 \\
\bottomrule
\end{tabular}}
\end{tabular}


==> tables/app_nl_mech_float.tex <==

\begin{table*}[!htbp]
\centering
\footnotesize
\setlength{\tabcolsep}{2.5pt}
\input{tables/app_nl_mech.tex}
\caption{\textbf{The later language edit is applied less often on every base and within every pair class.} Shares (\%) of outputs whose own field shows each edit, with prefix controls relative to $A$ alone in points and lavender rows naming the row groups.}
\label{tab:app-nl-mech}
\end{table*}


==> tables/app_nl_repair.tex <==


\begin{tabular}{@{}llcccccc@{}}
\toprule
\hlheadrow \hlhd{Mode} & \hlhd{$N$} & \hlhd{One call} & \hlhd{Equiv.} & \hlhd{Non-inf.} & \hlhd{B drop} & \hlhd{A drop} & \hlhd{Anch. $>$ mode, Holm} \\
\midrule
Anchored $B$ edit & 16 & 97.0 & 13 & 3 & \hlkey 0.3 & 0.0 & -- \\
 & 64 & 99.7 & 18 & 13 & \hlpass \hlbest{0.0} & 0.0 & -- \\
 & 256 & 100.0 & 18 & 18 & \hlpass \hlbest{0.0} & 0.0 & -- \\
 & 1024 & 100.0 & 19 & 18 & \hlpass \hlbest{0.0} & 0.0 & -- \\
\midrule
Plain $B$ edit & 16 & 95.8 & 14 & 6 & \hlfail 100.0 & 0.0 & 1 \\
 & 64 & 100.0 & 17 & 14 & \hlfail 96.3 & 0.0 & 1 \\
 & 256 & 100.0 & 19 & 18 & \hlfail 86.0 & 0.0 & 1 \\
 & 1024 & 100.0 & 19 & 18 & \hlfail 95.2 & 0.0 & 1 \\
\midrule
SPoT & 16 & 92.2 & 10 & 4 & \hlpass \hlbest{0.0} & 0.0 & 0.051 \\
 & 64 & 98.7 & 18 & 8 & \hlpass \hlbest{0.0} & 0.0 & 0.39 \\
 & 256 & 100.0 & 19 & 19 & \hlpass \hlbest{0.0} & 0.0 & 1 \\
 & 1024 & 100.0 & 19 & 19 & \hlpass \hlbest{0.0} & 0.0 & 1 \\
\midrule
Connector & 16 & 96.0 & 12 & 5 & \hlpass \hlbest{0.0} & 0.0 & 1 \\
 & 64 & 99.5 & 17 & 13 & \hlpass \hlbest{0.0} & 0.0 & 0.89 \\
 & 256 & 100.0 & 18 & 16 & \hlpass \hlbest{0.0} & 0.0 & 0.063 \\
 & 1024 & 100.0 & 18 & 16 & \hlpass \hlbest{0.0} & 0.0 & 0.78 \\
\bottomrule
\end{tabular}


==> tables/app_nl_repair_float.tex <==

\begin{table*}[tp]
\centering
\footnotesize
\setlength{\tabcolsep}{5pt}
\hlclip{\input{tables/app_nl_repair.tex}}
\caption{\textbf{Every mode improves language composition, but only unanchored editing erases the successor.} One call is median pair accuracy (\%), and drops are losses of standalone $A$ and $B$ in points.}
\label{tab:app-nl-repair}
\end{table*}


==> tables/app_transfer.tex <==

\begin{tabular}{@{}llcccc@{}}
\toprule
\hlgrouprow \multicolumn{6}{@{}l}{\emph{Qwen2.5-0.5B: $B$ trained on 3 or 4 predecessors, one more held out (27 folds), or one connector on 18 pairs (3 folds)}} \\
\hlheadrow \hlhd{Method} & \hlhd{Labels per pair} & \hlhd{Held out} & \hlhd{No training} & \hlhd{Gaining 10 points} & \hlhd{Trained pairs} \\
\midrule
anchored $B$ & 16 & \hlbest{9.4} & 5.7 & \hlbest{3/27} & \hlbest{72.9} \\
 & 64 & \hlbest{11.3} & 5.7 & \hlbest{5/27} & \hlbest{91.1} \\
 & 256 & \hlkey 10.4 & \hlkey 5.7 & \hlbest{4/27} & \hlkey \hlbest{90.4} \\
connector & 16 & 4.8 & 5.7 & 0/27 & 45.3 \\
 & 64 & 8.3 & 5.7 & 2/27 & 62.2 \\
 & 256 & 9.3 & 5.7 & 2/27 & 60.3 \\
connector, epochs $\times 2$ & 16 & 6.4 & 5.7 & 1/27 & 56.5 \\
 & 64 & 8.5 & 5.7 & 2/27 & 82.5 \\
 & 256 & \hlbest{10.6} & 5.7 & 3/27 & 82.9 \\
connector, all pairs & 16 & 3.0 & 5.7 & 0/27 & 17.5 \\
 & 64 & 3.4 & 5.7 & 1/27 & 20.0 \\
 & 256 & 7.7 & 5.7 & 2/27 & 52.3 \\
all pairs, epochs $\times 2$ & 16 & 4.1 & 5.7 & 1/27 & 25.6 \\
 & 64 & 7.1 & 5.7 & 1/27 & 31.7 \\
 & 256 & \hlkey 9.0 & 5.7 & 3/27 & \hlkey 72.4 \\
all pairs, rate 0.02 & 16 & 3.4 & 5.7 & 1/27 & 18.0 \\
 & 64 & 2.5 & 5.7 & 0/27 & 18.9 \\
 & 256 & 8.5 & 5.7 & 2/27 & 54.7 \\
\midrule
\hlgrouprow \multicolumn{6}{@{}l}{\emph{Single-pair edits at 8 labels, seed 1, other partners: median change (points), share gaining 10 points (\%)}} \\
\hlheadrow \hlhd{Edit} & \hlhd{Partners} & \hlhd{0.5B} & \hlhd{1.5B} & \hlhd{7B} & \hlhd{Gemma} \\
\midrule
anchored $B$ & other predecessors & 0.0, 7.4 & $-$0.3, 4.6 & 0.0, 4.6 & 0.0, 7.4 \\
anchored $A$ & other successors & $+$0.6, 9.3 & 0.0, 3.7 & $+$0.3, 5.6 & $+$0.1, 8.3 \\
\midrule
\hlgrouprow \multicolumn{6}{@{}l}{\emph{$A$ edits: change of $A$ after a pretrained successor}} \\
\hlheadrow \hlhd{Edit} & \hlhd{Successor} & \hlhd{0.5B} & \hlhd{1.5B} & \hlhd{7B} & \hlhd{Gemma} \\
\midrule
anchored, 8 labels & \sk{ID} & \hlbest{$-$10.0} & \hlbest{$-$31.7} & \hlbest{$-$9.1} & \hlbest{$-$19.4} \\
 & \sk{ADD} & \hlbest{$-$28.9} & \hlbest{$-$71.8} & \hlbest{$-$58.2} & \hlbest{$-$1.0} \\
plain, 8 labels & \sk{ID} & $-$96.6 & $-$96.7 & $-$84.4 & $-$96.7 \\
 & \sk{ADD} & $-$49.8 & $-$80.2 & $-$61.2 & \hlbest{$-$1.0} \\
anchored, 4096 labels & \sk{ID} & \hlbest{$-$55.7} & \hlbest{$-$14.6} & \hlbest{$-$1.3} & \hlbest{$-$12.3} \\
 & \sk{ADD} & \hlbest{$-$95.2} & \hlbest{$-$41.8} & \hlbest{$-$21.3} & \hlbest{$-$54.2} \\
plain, 4096 labels & \sk{ID} & $-$100.0 & $-$99.7 & $-$83.2 & $-$99.8 \\
 & \sk{ADD} & \hlbest{$-$95.2} & $-$84.0 & $-$71.2 & $-$71.1 \\
\bottomrule
\end{tabular}


==> tables/app_transfer_float.tex <==

\begin{table*}[!htbp]
\centering
\footnotesize
\setlength{\tabcolsep}{2.6pt}\renewcommand{\arraystretch}{1.25}
\hlclip{\input{tables/app_transfer.tex}}
\caption{\textbf{Repair gains stay mostly with the trained partners.} The panels report held-out partners (\%), other partners after a single-pair edit, and contexts followed by pretrained \sk{ID} or \sk{ADD} (changes in points). Rows marked all pairs are a post hoc check sharing one connector across 18 training pairs and count gaining pairs, with means (\%) over pairs of per-pair medians over three training seeds.}
\label{tab:app-transfer}
\end{table*}

